Can Large Time Delays Observed in Light Curves of Coronal Loops be Explained by Impulsive Heating?

The light curves of solar coronal loops often peak first in channels associated with higher temperatures and then in those associated with lower. The time delays between the different narrowband EUV channels have been measured for many individual loops and recently for every pixel of an active region observation. Time delays between channels for an active region exhibit a wide range of values, with maxima $>$ 5,000\,s. These large time delays make up 3-26\% (depending on the channel pair) of the pixels where a significant, positive time delay is measured. It has been suggested that time delays can be explained by impulsive heating. In this paper, we investigate whether the largest observed time delays can be explained by this hypothesis by simulating a series of coronal loops with different heating rates, loop lengths, abundances, and geometries to determine the range of expected time delays between a set of four EUV channels. We find that impulsive heating cannot address the largest time delays observed in two of the channel pairs and that the majority of the large time delays can only be explained by long, expanding loops with photospheric abundances. Additional observations may rule out these simulations as an explanation for the long time delays. We suggest that either the time delays found in this manner may not be representative of real loop evolution, or that the impulsive heating and cooling scenario may be too simple to explain the observations and other heating scenarios must be explored.

==> code_description_RL.tex <==

\section{DESCRIPTION OF SIMULATIONS}


To calculate the evolution of these loops we rely on two different hydrodynamic codes, the Naval Research Laboratory's Solar Flux Tube Model (NRLSOLFTM; \citealt{1982ApJ...255..783M}) and the Predictive Science One-dimensional Hydrodynamic Model (PSOHM; \citealt{2013ApJ...773...94M}).   NRLSOLFTM will be used to address the dependence of time lag on the heating magnitude, heating duration, loop length,  and abundances.  PSOHM will be used to investigate how area expansion impacts the time lag, which is not possible with the NRLSOLFTM.  We set up both models with many of the same parameters and initial conditions.  

Both models solve the following 1D
hydrodynamic equations along the length of a loop:

\begin{equation}
\frac{\partial \rho}{\partial t}
+\frac{1}{A}\frac{\partial}{\partial s}\left(A\rho v\right)=0, 
\label{eq-mass}
\end{equation}
%
\begin{equation}
\rho\left(\frac{\partial v}{\partial t}+v\frac{\partial v}{\partial s}\right)= 
 -\frac{\partial p}{\partial s}+\rho g_s 
 +\frac{1}{A}\frac{\partial}{\partial s}\left(A\nu\rho
\frac{\partial v}{\partial s}\right),
\label{eq-mom}
\end{equation}
%
\begin{multline}
\frac{\partial T}{\partial t}
+\frac{1}{A}\frac{\partial}{\partial s}\left(ATv\right)=
-(\gamma-2)\frac{T}{A}\frac{\partial}{\partial s}\left(Av\right)+ \\
\frac{(\gamma-1)T}{p}
\left[\frac{1}{A}\frac{\partial}{\partial s}\left(A
\kappa_\parallel\frac{\partial T}{\partial s}\right)
-n_en_p{Q(T)}+{H}\right],
\label{eq-energy}
\end{multline}
%
where $s$ is the length along the loop, $T$, $p$, and $v$ are
the plasma temperature, pressure, and velocity, $n_e$ and $n_p$
are the electron and proton number density (assumed to be
equal), and $\gamma=5/3$ is the
ratio of specific heats. The mass density for the        plasma
is $\rho=\frac{1+4f_\mathrm{He}}{1+2f_\mathrm{He}}m_pn_e$, where $m_p$ is the proton mass and $f_\mathrm{He}$ is the fraction of helium to hydrogen particles.
The plasma pressure is $p=\frac{2+3f_\mathrm{He}}{1+2f_\mathrm{He}}kn_eT$; \textbf{$k$ is Boltzmann's constant}.
The gravitational acceleration projected
along the loop is $g_s=\bhat\cdot{\bf g}$, where $\bhat$ is the
unit vector along the magnetic field ${\bf B}$. The Spitzer thermal conductivity coefficient is   $\kappa_\parallel(T)=C_0
T^{5/2}\,\text{[erg/cm/s/K]}$.
%, with $C_0= 9\times 10^{-7}$, and $T$ in $\text{[K]}$.

%[NOTE: We ran the NRL code with He abundance = 6.3\%, but not the PS code.  The above description of rho is not accurate for the NRL code.]

$H(s,t)$ is the coronal heating function.  In this investigation, the heating function will be
\begin{equation}
H(s,t) = H_0 + H_{\rm imp}g(t)
\end{equation}
where $H_0$ is a small background heating, applied uniformly and constantly, $H_{\rm imp}$ is the magnitude of the
impulsive heating that is also uniformly applied along the loop over a short time.  The time dependence of the impulsive heating event, $g(t)$, is a triangular pulse
defined as 
\begin{eqnarray}
g(t) = t/\delta  \hspace{0.5in} 0&<t\le&\delta \\
g(t) = (2\delta - t)/\delta \hspace{0.5in}\delta &< t\le&2\delta
\end{eqnarray}
where $\delta$ is the total duration of the impulsive heating. 


In the PSOHM, a uniform
kinematic viscosity $\nu$ is used to damp out waves, and is made
very small, corresponding to a diffusion time $L^2/\nu \sim
2{,}000\,\text{hours}$; this term is absent in NRLSOLFTM. 
When considering solutions with loop expansion, the loop
cross-sectional area, $A(s)$, is inversely proportional to the
magnitude of the magnetic field $B(s)$ measured along the loop.


The small values of $\kappa_\parallel$ at
low temperatures produce very steep gradients in temperature in
the transition region that are difficult to resolve in numerical
calculations. In NRLSOLFTM, a fine mesh is centered on the steepest temperature
gradient.   The location of this fine mesh is re-evaluated at each time step.  
In  PSOHM, in order to minimize the mesh resolution
requirements, we have developed special treatment of the thermal
conduction and radiation loss function to artificially broaden
the transition region at low temperatures
\citep{2009ApJ...690..902L} without significantly affecting the
coronal solution \citep{2013ApJ...773...94M}. 

In the above equations, $Q(T)$ represents the radiative loss function.  
We consider two
versions of the radiative loss function derived from the CHIANTI (version~7.1) 
atomic database
\citep{1997A&AS..125..149D,2013ApJ...763...86L}, one with coronal abundances
\citep[\texttt{sun\_coronal\_ext.abund},][]{1992ApJS...81..387F,2002ApJS..139..281L,1998SSRv...85..161G}
the other with photospheric abundances 
\citep[\texttt{sun\_photospheric\_2007\_grevesse.abund},][]{2007SSRv..130..105G},
both
using the CHIANTI collisional ionization equilibrium model \citep{2009A&A...498..915D}.
 These two radiative loss functions are shown in the lower panel of Figure \ref{fig_tresp_abun}.

All the loops will be semi-circular and perpendicular to the solar surface.   
For both models, we start the loops in a cool, tenuous steady state atmosphere with a transition region temperature.  Both models include a dense, cool chromosphere as a mass well for the solution.  Radiation is turned off at chromospheric temperatures.  

Finally, we have run a test case to compare the output of the two codes.  With identical loop length, heating functions, geometries, and radiative loss functions, we find near identical ($\pm$5\%) time lags in 
all channel pairs, even with different initial conditions, boundary conditions, and other simulation parameters such as $f_\mathrm{He}$ and $C_0$.


\begin{figure}
\begin{center}
\includegraphics[width=8cm]{Tresp_v1.eps}
\includegraphics[width=8cm]{Tresp_v2.eps}
\includegraphics[width=8cm]{Radloss_v2.eps}
\caption{Top: The temperature response curves of the four AIA channels used in this analysis plotted on a logarithmic scale and again with the responses normalized in order to highlight the breadth of the 335\,\AA\ response. Bottom: radiative
loss functions calculated using CHIANTI 7.1 with coronal or photospheric abundances.} 
\label{fig_tresp_abun} 
\end{center}
\end{figure}



